Extended mean flow analysis of the circular cylinder flow

A new eigenvalue analysis is developed and applied to the circular cylinder laminar flow configuration to investigate the various mechanisms at play in the nonlinear saturation of perturbations yielding to limit cycles for supercritical values of the Reynolds number. Unlike the mean-flow analysis, which only accounts for the interaction of the first-harmonic of the time-periodic flow with its mean-flow, the so-called extended mean-flow analysis also accounts for its interaction with the second-harmonic. The results reveal the existence of two eigenvalues both having a growth rate exactly equal to zero. The high-frequency eigenmode gives better estimations of the frequency and spatial structure of the first-harmonic than the marginal modes obtained with the mean-flow analysis, especially when the Reynolds number is increased.

==> Figures/cavity.tex <==
% Generated with LaTeXDraw 2.0.8
% Sat Nov 15 19:45:03 CET 2014
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{0.6} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-7.0)(24.0,4.5)
 %\psgrid(0,-6.0)(24.0,6)
 \definecolor{mygray}{rgb}{0.8,0.8,0.8}
 \definecolor{mylightgray}{rgb}{0.95,0.95,0.95}
 \psframe[framearc=0.1,dimen=outer,fillstyle=solid,fillcolor=mygray,linewidth=0.0cm,linecolor=mygray](4,-7)(8,0)
 \psframe[framearc=0.1,dimen=outer,fillstyle=solid,fillcolor=mygray,linewidth=0.0cm,linecolor=mygray](14,-7)(19,0)
 \psframe[dimen=outer,fillstyle=solid,fillcolor=mylightgray,linewidth=0.0cm,linecolor=mylightgray](19,-7)(24,0)
 \psframe[dimen=outer,fillstyle=solid,fillcolor=mygray,linewidth=0.0cm,linecolor=mygray](7.5,-7)(14.5,-6)
 \psframe[dimen=outer,fillstyle=solid,fillcolor=mygray,linewidth=0.0cm,linecolor=mygray](4,-7)(5,0)
 \psframe[dimen=outer,fillstyle=solid,fillcolor=mygray,linewidth=0.0cm,linecolor=mygray](18,-7)(19,0)
 \psframe[dimen=outer,fillstyle=solid,fillcolor=mylightgray,linewidth=0.0cm,linecolor=mylightgray](0,-7)(4,0)
 \psline[linewidth=0.04cm,linestyle=dashed,dash=0.16cm 0.16cm](0,0)(4,0)
 \psline[linewidth=0.04cm,linearc=0.25](4,0)(8,0.0)(8,-6)
 \psline[linewidth=0.04cm](8,-6)(14,-6)
 \psline[linewidth=0.04cm,linearc=0.25](14,-6)(14,0)(19,0)
 \psline[linewidth=0.04cm,linestyle=dashed,dash=0.16cm 0.16cm](19,0)(24,0)
 \psline[linewidth=0.02cm,linestyle=dashed,dash=0.16cm 0.16cm](24,0)(24,4.5)(0,4.5)(0,0)
 \psarc[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{<-}(11,-3.2){2.5}{-250}{30}
 \psplot[linewidth=0.01cm,algebraic,plotpoints=500]{8.5}{13.5}{0.035*x*sin(3*3.14*x/2)}
 \psline[arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(13.4995,0.32316)(13.5,0.324)
 %\psarc[linewidth=0.01cm](14.25,-0.25){4}{110}{175}
 %\psarc[linewidth=0.01cm](14.25,-0.25){3}{110}{175}
 %\psarc[linewidth=0.01cm](14.25,-0.25){2}{110}{175}
 \psline[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(-1.2,0)(-0.1,0.0)
 \psline[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(-1.2,0.7)(-0.1,0.7)
 \psline[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(-1.2,1.4)(-0.1,1.4)
 \psline[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(-1.2,2.1)(-0.1,2.1)
 \psline[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(-1.2,2.8)(-0.1,2.8)
 \psline[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(-1.2,3.5)(-0.1,3.5)
 \psline[linewidth=0.01cm,arrowsize=0.2cm 1.0,arrowlength=1.0,arrowinset=0.0]{->}(-1.2,4.2)(-0.1,4.2)
 \psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(0.0,-2.5)(4.0,-2.5)
 \psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(4.0,-2.5)(8.0,-2.5)
 \psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(14.0,-2.5)(19.0,-2.5)
 \psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(19.0,-2.5)(24.0,-2.5)
 \psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(19.0,0)(19.0,4.5)
 \usefont{T1}{ppl}{m}{n}
 \rput(-0.7,4.8){\LARGE $U_\infty$}
 \rput(0.8,2.5){\LARGE $\Gamma_{in}$}
 \rput(11,5){\LARGE $\Gamma_{top}$}
 \rput(24.8,2.5){\LARGE $\Gamma_{out}$}
 \rput(20.7,2.5){\LARGE $L_{top}=0.5$}
 \rput(15,-6){\LARGE $\Gamma_{wall,c}$}
 \rput(2,0.5){\LARGE $\Gamma_{slip,u}$}
 \rput(6,0.5){\LARGE $\Gamma_{wall,u}$}
 \rput(16,0.5){\LARGE $\Gamma_{wall,d}$}
 \rput(21,0.5){\LARGE $\Gamma_{slip,d}$}
 \rput(2,-2){\LARGE $L_{slip,u}=0.8$}
 \rput(6,-2){\LARGE $L_{wall,u}=0.4$}
 \rput(16.5,-2){\LARGE $L_{wall,d}=0.75$}
 \rput(21.4,-2){\LARGE $L_{slip,d}=0.75$}
\end{pspicture}
}

==> Figures/cyl.tex <==
% Generated with LaTeXDraw 2.0.8
% Sat Nov 15 19:45:03 CET 2014
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{0.65} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-6.2789063)(23.265625,6.2789063)
\definecolor{color71b}{rgb}{0.7215686274509804,0.7215686274509804,0.7215686274509804}
\psframe[linewidth=0.02,dimen=outer](19.975939,5.120312)(2.9559374,-5.499687)
\pscircle[linewidth=0.02,dimen=outer,fillstyle=solid,fillcolor=color71b](8.37,-0.29578125){0.51}
\psline[linewidth=0.01cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{->}(2.53,-0.29578125)(21.13,-0.29578125)
\psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(8.395937,0.98031247)(20.015938,0.98031247)
\psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(8.315937,2.9603126)(2.9559374,2.9603126)
\psline[linewidth=0.02cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<->}(4.975937,-0.2996875)(4.975937,-5.4396873)
\psline[linewidth=0.01cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.19cm 2.0,arrowlength=1.5,arrowinset=0.4]{<-}(8.37,5.8142185)(8.37,-6.1857815)
\usefont{T1}{ppl}{m}{n}
\rput(21.092812,0.81921875){\Large $\Gamma_{out}$}
\usefont{T1}{ppl}{m}{n}
\rput(13.8025,1.3503125){\Large $L_{o}=30$}
\usefont{T1}{ppl}{m}{n}
\rput(6.5,-2.9496875){\Large $L_{s}=20$}
\usefont{T1}{ppl}{m}{n}
\rput(5.6034374,3.4){\Large $L_{i}=20$}
\usefont{T1}{ppl}{m}{n}
\rput(11.058281,5.619219){\Large $\Gamma_{top}$}
\usefont{T1}{ppl}{m}{n}
\rput(10.812344,-5.980781){\Large $\Gamma_{bottom}$}
\usefont{T1}{ppl}{m}{n}
\rput(1.8928125,0.6103125){\Large $\Gamma_{in}$}
\usefont{T1}{ppl}{m}{n}
\rput(20.792812,-0.68078125){\Large $x$}
\usefont{T1}{ppl}{m}{n}
\rput(8.092813,6.019219){\Large $y$}
% double spring sketch
%\psline[linewidth=0.03](7.972593,-1.1810937)(7.972593,-1.5410937)(8.287619,-1.6693714)(7.78,-1.837842)(8.3,-2.0063126)(7.804762,-2.1747835)(8.027619,-2.251361)(8.027619,-2.4810936)
%\psline[linewidth=0.03cm](8.0,-2.8010938)(8.74,-2.8010938)
%\psframe[linewidth=0.01,dimen=outer,fillstyle=solid,fillcolor=color71b](8.74,-2.8210938)(8.0,-2.9810936)
%\psline[linewidth=0.03](9.24,-0.02109375)(9.54,-0.02109375)(9.678165,0.25890625)(9.840588,-0.24109375)(10.039104,0.25890625)(10.178237,-0.24109375)(10.288016,0.016970767)(10.64,0.01890625)
%\psline[linewidth=0.03cm](10.94,0.01890625)(10.94,-0.60109377)
%\psframe[linewidth=0.01,dimen=outer,fillstyle=solid,fillcolor=color71b](11.12,0.01890625)(10.96,-0.60109377)
%\psline[linewidth=0.03cm](8.38,-0.76109374)(8.38,-1.1810937)
%\psline[linewidth=0.03cm](8.72,-1.1610937)(8.72,-1.9410938)
%\psline[linewidth=0.03](8.62,-1.8010937)(8.62,-2.0410938)(8.86,-2.0410938)(8.86,-1.8010937)
%\psline[linewidth=0.03cm](8.74,-2.0410938)(8.74,-2.5010939)
%\psline[linewidth=0.03cm](7.96,-1.1810937)(8.74,-1.1810937)
%\psline[linewidth=0.03cm](8.02,-2.50)(8.72,-2.50)
%\psline[linewidth=0.03cm](8.38,-2.4810936)(8.38,-2.8010938)
%\psline[linewidth=0.03cm](9.24,-0.60109377)(10.0,-0.60109377)
%\psline[linewidth=0.03](9.86,-0.46109375)(10.12,-0.46109375)(10.12,-0.74109375)(9.86,-0.74109375)
%\psline[linewidth=0.03cm](10.12,-0.60109377)(10.64,-0.60109377)
%\psline[linewidth=0.03cm](9.24,-0.02109375)(9.24,-0.62109375)
%\psline[linewidth=0.03cm](10.64,0.01890625)(10.64,-0.60109377)
%\psline[linewidth=0.03cm](8.88,-0.30109376)(9.22,-0.30109376)
%\psline[linewidth=0.03cm](10.64,-0.30109376)(10.92,-0.30109376)
\usefont{T1}{ppl}{m}{n}
\rput(7.5,0.3){\Large $\Gamma_{cyl}$}
\end{pspicture} 
}


